Deep Learning-based Embedded Intrusion Detection System for Automotive CAN

Rising complexity of in-vehicle electronics is enabling new capabilities like autonomous driving and active safety. However, rising automation also increases risk of security threats which is compounded by lack of in-built security measures in legacy networks like CAN, allowing attackers to observe, tamper and modify information shared over such broadcast networks. Various intrusion detection approaches have been proposed to detect and tackle such threats, with machine learning models proving highly effective. However, deploying machine learning models will require high processing power through high-end processors or GPUs to perform them close to line rate. In this paper, we propose a hybrid FPGA-based ECU approach that can transparently integrate IDS functionality through a dedicated off-the-shelf hardware accelerator that implements a deep-CNN intrusion detection model. Our results show that the proposed approach provides an average accuracy of over 99% across multiple attack datasets with 0.64% false detection rates while consuming 94% less energy and achieving 51.8% reduction in per-message processing latency when compared to IDS implementations on GPUs.

==> background.tex <==
\iffalse
\section{Background and Related Work}\label{sec:background}
\subsection{Controller Area Network}
In-vehicle networks enable distributed ECUs to exchange control and data messages to achieve the global functions of the vehicle. 
Multiple protocols are used in vehicular systems to cater to different functions based on their criticality and to optimise the cost of E/E systems. 
CAN~\cite{CanBosch} and CAN-FD~\cite{hartwich2012can} continues to be the most widely used protocol today due to its lower cost, flexibility and robustness. 
Figure~\ref{fig:1} illustrates the bit-field definition of CAN data frame, with each segment providing some function in the network operation. %, as
\iffalse
Each bit-field within the CAN frame serves a specific purpose: start of frame (SOF) bit indicating a start of a new message, remote transmission request (RTR) bit to request information from another ECU, acknowledge (ACK) field to indicate errors in frame and the cyclic redundancy check (CRC) field carrying a CRC value. 
The CAN ID (11 bit base, 29 bit extended format) is a unique identifier assigned to each message and by extension, defines its priority for transmission on the shared bus.
The message itself is contained in the data field.
\fi
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{figures/CANbus.pdf}
  \caption{Frame format of an extended frame CAN message. In case of a standard CAN message, the ID field contains the 11 bit identifier.}
  \label{fig:1}
  \vspace{-10pt}
\end{figure}
The broadcast CAN bus uses a bit-wise arbitration method to control medium access to the bus using the CAN ID allocated to each message. 
CAN also supports multiple data rates (125\,Kbps to 1\,Mpbs) and multiple modes of operation (1-wire, 2-wire) to cater to a range of critical and non-critical functions in vehicles. 
Despite this robustness, CAN is inherently insecure: there is no built-in mechanism in the network to authenticate the transmitter, receiver or the message content itself~\cite{8658720}.  
This makes CAN vulnerable to simple and efficient attacks like message sniffing, fuzzing, spoofing, replay attacks and Denial of Service (DoS) attacks.~\cite{mukherjee2016practical,enev2016automobile,koscher2010experimental,palanca2017stealth}.
However, physical access to CAN bus is required for such attacks and thus detecting intrusions on CAN network is of key interest. 

\subsection{IDSs for CAN}
Researchers have explored various techniques to detect intrusions in CAN bus.
These can be broadly classified into flow-based, payload-based and hybrid schemes that combine the flow-based and payload-based techniques~\cite{al2019intrusion}.
Flow-based approaches extract identifiable traits like message frequency and/or interval for the network and use these to determine abnormal activity on the network~\cite{ling2012algorithm}.\iffalse vuong2015performance \fi
Payload-based schemes use the information in the CAN frames to detect abnormal sequences of instructions or data~\cite{narayanan2015using}. \iffalse stabili2017detecting \fi
Hybrid scheme uses both the timing information and the CAN frame fields to create a more holistic view, allowing them to extract specific signatures of transmitting ECUs, receiving ECUs and messages~\cite{weber2018embedded,vasistha2017detecting}. \iffalse ,8688625 \fi 
\iffalse
For instance, fingerprint-based approach uses low-level electrical signal levels and timing of signals in relation with the message contents to identify potential intrusions when large deviations are observed~\cite{cho2016fingerprinting}.\iffalse ,cho2017viden \fi
Parameter monitoring-based techniques extract message-level frequency and timing characteristics for different fields or specific messages, like offset ratio and timing in case of a remote transmission frame, to identify potential intrusions~\cite{lee2017otids}.
Researchers have also proposed the use of entropy of the network traffic as a method to identify abnormal conditions and intrusions~\cite{wu2018sliding}.
\fi
Such approaches are further generalised by machine learning based techniques, including classification approaches, deep learning based schemes and sequential techniques. 
%\subsection{ML-based IDS}

Most ML-based approaches fall under the hybrid scheme, utilizing both the content of the message frame and their timing/frequency characteristics to achieve better detection. 
In~\cite{alshammari2018classification}, the authors use the offset ratio and time intervals between remote requests to classify DoS and fuzzy attacks using an Support Vector Machine classifier. 
Tree-based approaches explored by~\cite{yang2019tree} uses CAN IDs and data segment contents as input features to tree-based classifiers like decision trees, random forests and others. 
In~\cite{song2020vehicle}, the authors propose a reduced inception net architecture for IDS which uses deep convolutional neural networks. 
The authors show that the ML architecture can achieve over 99\% accuracy across DoS, fuzzing and spoofing attacks.
The authors used a dataset captured from actual vehicle for training and testing their model, which has been shared with the community for further research.
Since the dataset covers multiple attack modes with actual CAN messages, we use the same dataset to train and evaluate our proposed architecture. %\todo[inline]{\textcolor{darkgreen}{So these guys use this paper as their reference for the dataset...So should i cite the link at which the dataset is?}Cite the dataset here}
In~\cite{tariq2020cantransfer}, the authors use a convolutional long-short-term memory (LSTM)-based architecture with transfer learning to enable faster adaptation for newer attacks. 
The model uses entire CAN frames as its input feature and offered over 95\% detection accuracy across DoS, fuzzing and replay attacks when tested with their propitiatory dataset. %\todo[inline]{Is it the same dataset? what is the accuracy they claim for each of these ML IDSs?\textcolor{darkgreen}{They built their onw dataset from two vehicles and they don't report their accuracies individually on the three attacks but as an average where there precison, recall and F1 values are around 95\%}}
A variation of this approach is described in~\cite{desta2020mlids,hanselmann2020canet} where the authors propose the use of individual LSTMs that are trained to individual CAN IDs. 
In~\cite{seo2018gids}, authors present a GAN-based IDS trained using CAN IDs and achieve an average accuracy of 97.5\% across the DoS, Fuzzy and spoofing attacks. 
%Intrusion Prevention Systems have also been proposed in the context for CAN. 
In~\cite{de2021efficient}, the authors use an iForest anomaly detection algorithm to detect fuzzing and spoofing (RPM \& Gear) attacks and marks the message as an error preventing its propagation to other ECUs; however this can cause multiple messages to be dropped from the bus in case of false positives or DoS attacks.  
%They discard a message that is identified as an intrusion before it is transmitted to the ECUs. 
%However, this approach can cause all the messages in the bus to dropped in case of DoS attacks raising safety concerns.
In most cases, the inference models are deployed through powerful GPUs to achieve line rate detection on actual CAN bus (using CAN datasets), quantifying detection accuracy and processing latency (in batch-style operation).
%Most of the works focus only on accuracy of their implementations; processing latency \& power consumption are crucial metrics overlooked in the above papers. 
%We focus on the accuracy, processing latency, power consumption \& resource utilisation metrics of our implementation, presenting a wholesome analysis.
Our approach aims at integrating the ML accelerators as a standard peripheral within a traditional ECU, with optimisations to achieve high accuracy and throughput, at much lower power consumption compared to traditional GPU implementations.
\iffalse
Hence we quantify the detection accuracy and processing latency (in batch and per-message cases), as well as an analysis on the power consumption across multiple deployment modes and scalability of the integrated approach. 
\fi
\iffalse
\subsection{Machine Learning on FPGAs}
While GPUs have been the target device of choice for most machine learning inference applications, FPGAs have shown great promise in recent years. 
Early efforts of deep learning accelerators on FPGAs suffered from limited on-chip memory resources, requiring most weights and biases to be stored off chip, resulting in performance penalties compared to GPU implementations~\cite{xiao2017exploring}.
Furthermore, such accelerators had to be custom built and optimised while also managing efficient data movement between off-chip memory and interfaces, requiring significant hardware expertise. 
Recent approaches for deploying deep learning inference on FPGAs have reduced this barrier, while still providing significant performance and energy benefits over GPUs~\cite{wang2019survey, BLAIECH2019331, wang2016dlau}.
Tool-chains like DNN-Weaver~\cite{sharma2016dnnweaver}, LUTNET~\cite{wang2019lutnet} and FINN~\cite{umuroglu2017finn}  can efficiently map high level representations of ML models for executing on pre-composed hardware accelerators or into fully custom accelerators. 
%Traditional ML models use native data representation formats (float, int) which are then handled by GPUs.
These tools also optimise native data representation formats (float, int)  through pruning and quantisation to reduce computational complexity and memory footprint required by the implementations.
The loss of accuracy in such optimisations is addressed by augmenting training steps  and/or post-quantisation fine-tuning. % that can minimise the loss in accuracy which could otherwise occur. 
%Frameworks like DNN-Weaver~\cite{sharma2016dnnweaver}, LUTNET~\cite{wang2019lutnet} and FINN~\cite{umuroglu2017finn} allow designers to compose FPGA-optimised quantised neural network accelerators from high level representations, lowering the barrier for using FPGA-based ML accelerators. 
With some hardware expertise, these frameworks will allow every layer of the network to be optimised (including weights, biases and activation functions) and right-sized  (down to 1-bit in case of FINN) with minimal impact on accuracy, generating energy efficient high-performance implementations, which can then be connected as slave accelerators in an embedded design or used as standalone accelerators. 
%Binarised neural networks (BNNs) generated through the FINN framework  
Alternatively, vendor flows like Vitis-AI from Xilinx~\cite{xilinxvitis} maps a pre-trained network onto a selection of pre-composed configurable deep-learning processing units (DPUs)~\cite{xilinxdpu} on the hardware, lowering the barrier for using FPGA-based ML accelerators.
The Vitis-AI flow quantizes and (optionally) fine-tunes the pre-trained model to generate the hardware accelerator model along with its drivers and APIs for offloading computations to it from a host code. 
While not fully optimised as a custom implementation generated through FINN, the Vitis-AI flow offers a compelling alternative to the GPU flow, and hence, in this paper, we utilise the Vitis-AI flow to design and deploy our IDS accelerator on the hybrid Zynq Ultrascale+ device. 
FPGAs are gaining momentum in the automotive domain, with prior research having explored acceleration of real-time complex algorithms for vision-based advanced driver assistance systems (ADAS) and using network interface extensions to augment ECU functionality and security~\cite{shreejith2018smart}.
FPGA-based ECUs architectures have also been explored to enable custom capabilities while maintaining complete AUTOSAR compliance~\cite{fons2012fpga}.
Automotive suppliers and vendors have also explored hybrid FPGA-based ECUs for improved functional consolidation and reliability~\cite{BoschMS6}. 
Network anomaly detection (bit-timing~\cite{zhou2019btmonitor}, transmission timing~\cite{yang2020identify}) models and probabilistic attack models~\cite{8987605} to detect spoofing attacks on CAN bus have leveraged FPGA platforms for improved latency and detection performance.  
%In, the authors adopt a Bayesian network model to detect spoofing attacks on a CAN bus using the hybrid Zynq FPGA as the implementation platform.
%Other works have also explored custom ML models on FPGAs that use transmission timing analysis and bit-time discrepancies~\cite{zhou2019btmonitor} in CAN frames to identify authentic ECUs in the network.
With the rising computational complexity in vehicles, it is expected that hybrid FPGA based ECUs will gain more traction for complex vehicular functions. 
Our approach aims at a generic IDS implementation that can cater towards multiple attack vectors through a dedicated accelerator attached as a slave peripheral device to the ECU, mimicking an off-the-shelf ECU architecture.
\fi
\fi

